How Close and How Much? Linking Health Outcomes to Built Environment Spatial Distributions

Built environment features (BEFs) refer to aspects of the human constructed environment, which may in turn support or restrict health related behaviors and thus impact health. In this paper we are interested in understanding whether the spatial distribution and quantity of fast food restaurants (FFRs) influence the risk of obesity in schoolchildren. To achieve this goal, we propose a two-stage Bayesian hierarchical modeling framework. In the first stage, examining the position of FFRs relative to that of some reference locations - in our case, schools - we model the distances of FFRs from these reference locations as realizations of Inhomogenous Poisson processes (IPP). With the goal of identifying representative spatial patterns of exposure to FFRs, we model the intensity functions of the IPPs using a Bayesian non-parametric viewpoint and specifying a Nested Dirichlet Process prior. The second stage model relates exposure patterns to obesity, offering two different approaches to accommodate uncertainty in the exposure patterns estimated in the first stage: in the first approach the odds of obesity at the school level is regressed on cluster indicators, each representing a major pattern of exposure to FFRs. In the second, we employ Bayesian Kernel Machine regression to relate the odds of obesity to the multivariate vector reporting the degree of similarity of a given school to all other schools. Our analysis on the influence of patterns of FFR occurrence on obesity among Californian schoolchildren has indicated that, in 2010, among schools that are consistently assigned to a cluster, there is a lower odds of obesity amongst 9th graders who attend schools with most distant FFR occurrences in a 1-mile radius as compared to others.

==> Extra_tex_files/extrafigures.tex <==
\begin{comment}
\begin{figure}[H]
    \centering
    \includegraphics[width = .7 \textwidth]{probmap_density1.png}
    \caption{(Top) Spatial map of the probability of co-clustering with a reference school denoted by a star. Probabilities are color-coded with darker colors indicating larger probabilities within each of the 4 probability intervals considered, (0,0.25], (0.25,0.5]. (0.5,0.75] and (0.75, 1]. (Bottom) Estimated density function of the FFRs distance to the school for the cluster to which the reference school is assigned.}
    \label{fig:probmap1}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width = .7 \textwidth]{probmap_density2.png}
    \caption{Spatial map of the probability of co-clustering with a reference school denoted by a star. Probabilities are color-coded with darker colors indicating larger probabilities within each of the 4 probability intervals considered, (0,0.25], (0.25,0.5]. (0.5,0.75] and (0.75, 1]. (Bottom) Estimated density function of the FFRs distance to the school for the cluster to which the reference school is assigned.}
    \label{fig:probmat2}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width = .7 \textwidth]{probmap_density3.png}
    \caption{Spatial map of the probability of co-clustering with a reference school denoted by a star. Probabilities are color-coded with darker colors indicating larger probabilities within each of the 4 probability intervals considered, (0,0.25], (0.25,0.5]. (0.5,0.75] and (0.75, 1]. (Bottom) Estimated density function of the FFRs distance to the school for the cluster to which the reference school is assigned.}
    \label{fig:probmat3}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width = .7 \textwidth]{probmap_density4.png}
    \caption{Spatial map of the probability of co-clustering with a reference school denoted by a star. Probabilities are color-coded with darker colors indicating larger probabilities within each of the 4 probability intervals considered, (0,0.25], (0.25,0.5]. (0.5,0.75] and (0.75, 1]. (Bottom) Estimated density function of the FFRs distance to the school for the cluster to which the reference school is assigned.}
    \label{fig:probmat4}
\end{figure}
\end{comment}

==> Extra_tex_files/extratext.tex <==
%Trying to channel the below comment into the above paragraph
%we can use a DP process prior and the kernel mixing representation to model non-parametrically each of the f_i's.
%If we want to cluster the f_i's, then we would think of using an additional hierarchy in our model, which is why we go for the nested DP.
 \begin{comment}
To begin, consider the estimation of a single school's representative density function in the absence of data from any other school.  In order to estimate this function non-parametrically, we could use a Dirichlet Process (DP) \cite{gelman2013bayesian,ferguson1973bayesian} to estimate the appropriate distribution or mixing measure, $G$, with which to estimate the $f_i(r)$. This approach corresponds to the following expression:
\begin{align*}
    f_i(r) &= \int \mathcal{K}(r|\bm{\theta})G(\bm{\theta})\\
    G & \sim DP(\alpha,G_0).
\end{align*}
Where $\mathcal{K}$ is a known parametric kernel with parameters $\bm{\theta}$, $DP(\alpha,G_0)$ denotes a DP prior with concentration parameter $\alpha>0$ and base measure $G_0$ which is typically set to be some known parametric distribution. The above model would cluster distances to some local parametric distribution, with cluster specific parameters, so that the resulting function would combine information across space, incorporating local features into the overall density estimate. 
\par 
In order to build upon this approach so that information is combined both across distance and schools, we utilize the NDP, which allows for the estimation of a school specific mixing measure $G_i$. Now, analogous to how similar distances may inform the same parametric cluster density in the simple example above, similar school densities may inform a school-cluster density:
\begin{align*}
f_i(r) &= \int \mathcal{K}(r|\bm{\theta})dG_i(\bm{\theta})\\
    G_i &\stackrel{iid}{\sim} Q \\
    Q &\equiv DP(\alpha,DP(\beta,G_0)).
\end{align*}
Where $Q$ is defined as a NDP with two concentration parameters,$\alpha>0,\beta>0$ and $G_0$ remains a parametric base measure.
\par 
\end{comment}





\begin{comment}
\subsection*{California Model Specification}
In our application of the above NDP formulation to the CA high school data we truncate the number of cluster components at $K=35$ and within cluster components $L=30$, similar to previous work on a dataset of similar size \cite{rodriguez2008nested}. Following the example and direction set by \cite{rodriguez2008nested,ishwaran2001gibbs} further,  we use an informative Gamma prior on $\alpha$ and $\rho$ centered at 1 as is common in the literature. We run the Gibbs sampler for 250,000 iterations using the \texttt{bendr}\footnote{(v0.1.0, https://github.com/apeterson91/bendr)} package, saving the last 10000 iterations thinned by three for a total of 3,333 posterior samples. This number is chosen by the Raftery diagnostic\cite{raftery1995number} to ensure accurate quantile estimation, with the thin chosen to reduce auto-correlation seen in the inference of the $\alpha$ and $\rho$ parameters. The aforementioned concentration parameters were used to assess convergence via trace-plot and Geweke statistic\cite{geweke1991evaluating}, since the varying cluster parameters may exhibit label-switching\cite{gelman2013bayesian}.  The full model specification can be found below, with posterior estimates and figures displayed in Section 4.1.
\begin{align*}
    r'_{ij}|n_j &\sim f_i(r') \quad j=1,...,782,i=1,...n_j\\
    f_i(r') &= \int \mathcal{N}(r'|\mu,\sigma^2) dG_i((\mu,\sigma^2))\\
    G_i &\sim Q\\
    Q &= \sum_{k=1}^{K=35}\pi^*_k \delta_{G_j^*}(\cdot)\\
    G_k^* &= \sum_{l=1}^{L=30} w^*_{lk}\delta_{(\mu^*_{lk},\sigma^{*2}_{lk})}(\cdot)\\
    \alpha &\sim \text{Gamma}(10,10)\\
    \rho &\sim \text{Gamma}(10,10)\\
    (\mu_{lk},\sigma^{2}_{lk}) &\sim \mathcal{N}(0,\sigma^{2}_{l,k})\times \text{Inv-}\chi^{2}(1,1)
\end{align*}
\end{comment}



==> Extra_tex_files/removed_estimation_simulation.tex <==
% This section currently removed from paper - keeping the text just in case we need it later
\begin{comment}
\subsection{Estimation}

\textcolor{blue}{Not sure if this text should be included or not. If it is included or maybe is added to the supplementary material, I suggest being careful not using symbols that have been already used before. This would make following very hard for a reader if the same symbols are used twice to mean different things.}
To further clarify the relationship between school cluster membership, density, and parameter estimation, we elucidate the sampling scheme for the pertinent parameters. First, define $\zeta_j$ to be the latent membership indicator of the $j$th school as signed to a unique mixing measure: $\zeta_j = k$ if $G_j = G_k^*$. Similarly,  if we let $\xi_{ij} = l$ denote the latent membership indicator of the distance $r_{ij}$ to a specific parameter mixture component, $\theta^*_{lk}$, within mixing measure $G^*_k$, we're able to update both parameters via Gibbs' steps\cite{rodriguez2008nested}:

\begin{align*}
    p(\zeta_j=k|\cdot) &\propto \pi^*_k \prod_{i=1}^{n_j}\sum_{l=1}^{L}  w^*_{lk}\mathcal{K}(r_{ij}|\theta^*_{lk})\\
    p(\xi_{ij}=l|\zeta_j,\cdot) &\propto w^*_{l,\zeta_j}\mathcal{K}(r_{i,\zeta_j}|\theta^*_{l,\zeta_j}).
\end{align*}

Following estimation of school and school-distance latent indicators, weights $\pi^*_k$ and $w^*_{k,l}$ can be updated by generating: 
\begin{align*}
\pi^{*}_k &= u_k\prod_{s=1}^{k-1} (1-u^{*}_s) \qquad u_k^{*}|\cdot \sim \text{beta}(1+m_k, \alpha + \sum_{s=k+1}^{K} m_s)    \\
w^{*}_{k,l} &= v_{k,l}\prod_{s=1}^{l-1} (1-v^{*}_{k,s}) \qquad v_{k,s}^{*}|\cdot \sim \text{beta}(1+n_{k,l}, \rho + \sum_{s=l+1}^{L} n_{s,l}),
\end{align*}
where $m_k,n_{k,l}$ indicate the number of schools or school-distances assigned to the $k$th cluster or the $k,l$th within-cluster mixture component, respectively.
\par Subsequent to weight updates, updates of the parameters $\theta^*_{lk}$ can be made via conjugate or Metropolis-Hastings updates using the following posterior expression, which shows how data from differing schools will potentially pool to inform the cluster parameters:

\begin{align*}
    p(\theta^*_{lk}|\cdot) &\propto G_0(\theta^*_{lk})\times \prod_{\{i,j| \zeta_j = k, \xi_{ij} = l \} } \mathcal{K}(r_{ij}|\theta^*_{lk}).
\end{align*}
 Finally, to update $\bm{\beta}$ in the regression component of the model, the following proportional posterior function incorporating prior information $p(\bm{\beta})$ is used:
$$
p(\bm{\beta}|\cdot) \propto \prod_{j=1}^{J} \exp \{ \{n_jx_j^{T}\bm{\beta} \}\} \exp \{ -\exp \{ \bm{x}_j^{T}\bm{\beta}  \} \} p(\bm{\beta}) 
$$



\section{Simulations:}

To compare the efficacy of our NDP model to a more naive approach, we simulate distances $\{r_{ij}\}$ from one of three intensity functions (Figure \ref{fig:simulated_densities} (Top)) that are themselves composed of two-three simpler densities. The exact specification for how these data are simulated can be found in the supplementary material. Our comparison model will be a simple  finite hierarchical mixture model (FHMM) where the number of within-cluster components used to estimate the underlying intensities, $L$, is fixed at $L=4$ and $K$ the number of possible intensities to which a simulated school can be associated is varied across model fittings from 2 to 8. In the following FHMM framework we use similar notation to highlight the similarities between the two approaches:
\begin{align*}
	r_{ij} | \zeta_j &\stackrel{iid}{\sim} f_{\zeta_j}(r) \quad i = 1,..,n_j; j=1,...,J\\
	f_k(r) &= \sum_{l=1}^{4}w_l\mathcal{K}(r_{i,\zeta_j}|\theta_{l, \zeta_j})\quad k = 1,...,K\\
	\bm{\zeta} &\sim \text{Multinomial}(\pi_1,...,\pi_K)\\	
	\bm{\pi} &\sim \text{Dirichlet}(\bm{\omega})\\
	\bm{w} &\sim \text{Dirichlet}(\bm{\nu})\\
	\theta_{lk} &\sim p(\theta).\\
\end{align*}
In our simulations' model fittings we fit the FHMM using a normal kernel $\mathcal{K}$ in addition to a normal prior $\theta_{lk}=(\mu_{lk},\sigma^2{lk}) \sim N(1,\sigma^2)\text{Inv}\chi^{2}(1,1)$ so that conjugate updates can ease computation. Consequently, we transform the simulated distances through the probit function to put them on the correct domain. Hyperparameters for the Dirichlet distributions are all set to be 1; i.e. $\bm{\nu}=\bm{\omega}=\bm{1}$ so as to have a non-informative prior. The NDP model uses the same normal-inverse chi-square base measure as the FHMM, while the concentration parameters $\alpha = \rho = 1$ in accordance with standard simulation settings in this area \cite{rodriguez2008nested,ishwaran2001gibbs,gelman2013bayesian} and emphasizing an \textit{a priori} model skepticism towards introducing many new clusters. Our strategy in setting these priors is meant to emulate an analyst's typical approach when fitting these models in the absence of strong prior information \cite{gelman2013bayesian,rodriguez2008nested}.
\par We seek to identify any advantage gained from using the NDP over the FHMM and to that end we fit each model to 10(can do more later) datasets consisting of 50 groups of distances each generated under the 3 intensities described above for a total of 150 groups. We then vary K, the number of potential clusters under the FHMM, to reflect the fact that \textit{a priori} an analyst using the FHMM does not know what number of components is the correct number to use. We set the the truncation number for the analogous NDP component to be 10 for the number of cluster components and 4 for within cluster components mainly for computational convenience, but note that a higher truncation could be used with equivalent results.
\par In order to compare these models we calculate two different loss functions. The first compares the true and estimated clustering membership through the membership indicators - $\zeta_j,\hat{\zeta}_j$ - and the second calculates the quadratic loss between the true and estimated probability of co-clustering two simulated schools: $p_{l,j},\hat{p}_{l',j'}$. The first loss function was used in the original development of the NDP as well as in other Bayesian classification models by Binder, Lau \& Green, while the second is used here as a familiar benchmark\cite{rodriguez2008nested,lau2007bayesian,binder1978bayesian}.
\begin{align*}
    &\sum_{(j,j'): j< j' \leq J} I(\zeta_j=\zeta_{j'},\hat{\zeta_j}\neq\hat{\zeta_{j'}}) + I(\zeta_j\neq\zeta_{j'},\hat{\zeta_j}=\hat{\zeta_{j'}}) \tag{Binder, Lau \& Green}\\
    &\sum_{(l,j),(l',j') } (\hat{p}_{l,j} - p_{l',j'})^2 \quad l< j < J;\quad  l'< j' < J. \tag{ Quadratic Loss }
\end{align*}    


We present the results from these simulations in Figure \ref{fig:simulated_densities} (Bottom) and Table \ref{tab:simulations}. Figure \ref{fig:simulated_densities} shows the mean and 95\% confidence interval for each model across the differing values of $K$ and Table \ref{tab:simulations} shows the numerical values for the setting in which the FHMM has the same number of density function cluster components, $K$ as the data were simulated under.
	
\begin{figure}[H]
    \centering
    \includegraphics[width = .85 \textwidth ]{figures/demo_intensities.png}
    \includegraphics[width = .75 \textwidth ]{plot1.png}
    \caption{(Top) Generative Intensities, (Bottom) Simulation Model Comparison}
    \label{fig:simulated_densities}
\end{figure}
\begin{table}[H]
\centering
\begin{tabular}{llcc}
\hline
Loss Function &  & FHMM & \multicolumn{1}{c}{NDP} \\ 
\hline
Green \& Lau  & mean  & $3231.5$ & $1705.5$ \\
 & sd  & $\phantom{0}203.8$ & $\phantom{0}336.5$ \\
Quadratic & mean  & $2605.8$ & $\phantom{0}373.2$ \\
 & sd  & $\phantom{0}120.6$ & $\phantom{0}127.0$ \\
\hline 
\end{tabular}
\caption{Comparison in Loss Functions between the FHMM and NDP when the FHMM has the correct number of cluster components}
\label{tab:simulations}
\end{table}

\par The results from our simulations show a clear advantage for the NDP model, with both the mean quadratic and mean Green \& Lau classification error consistently lower than the corresponding FHMM error across $K$. Looking specifically at the case where $K=3$ in Table \ref{tab:simulations}, we see that the NDP Green \& Lau error is about half of the FHMM error and the mean quadratic loss is a whole order of magnitude lower. 
\par Much of the advantage the NDP demonstrates can be attributed to the model's conservative approach towards incorporating new clusters. That is to say, that since the naive approach places uniform weights on the within cluster components \textit{a priori}, there is considerable efficiency gained by the NDP's more ``skeptical'' approach which decreases the amount of weight placed on each subsequent mixture component according to the stick breaking rule in (2). This is especially useful in a setting such as this where there is only enough information to justify inclusion of two or three within cluster components.
\end{comment}


\begin{comment}
The intensity functions as used in the simulations are composed as follows:
\begin{align*}
f_1(r) &= (\frac{1}{2}\text{Beta}(r|1,8) + \frac{1}{2}\text{Beta}(d|6,1)), \\
f_2(r) &= (\frac{1}{5}\text{Beta}(r|3,2) + \frac{2}{3}\text{Beta}(r|3,1) + \frac{2}{15}\text{Beta}(d|1,1))\\
f_3(r) &= (\frac{1}{2}\text{Beta}(r|8,2) + \frac{1}{2}\text{Beta}(r,30,50))    
\end{align*}
where $\pi$Beta($r,\alpha,\beta)$ indicates a beta density evaluated at $r$  with shape parameters $\alpha, \beta >0$ weighted by $\pi \in [0,1]$.

\end{comment}

==> Paper_Sections/Data.tex <==
\subsection{Data sources and study sample}
\label{sec:Data_sources}
Each spring, public schools in the State of California collect data on the fitness status of pupils in 5th, 7th and 9th grade, as part of a state mandate, using the Fitnessgram battery. The Cooper Institute's sex-, age- and height-specific standards for body weight are used to classify each child as "meeting the standard", "needs improvement", or "needs improvement, high risk", which correlate to normal, overweight, and obese classifications. We use the last two of these as "not meeting the standard", and use the term obesity henceforth when referring to this outcome. Fitnessgram data are available through the California Department of Education (CDE) website (https://www.cde.ca.gov/ds/). In our analysis, we use data collected during academic year 2009-2010 on 9th graders only, since high school youth are more likely to be exposed to the food environment surrounding their school (e.g., students may leave the campus for lunch). 

Data on school-level characteristics are also available from the CDE website (see Table \ref{tab:CA_descriptive}), and, importantly, so is the geocode of the school. School geocodes were used for two purposes. First, the geocodes were used to link schools to census tract level covariates. Second, the school geocodes were used to calculate the distances between the school and the geocoded location of each FFR in California. FFRs were identified from the National Establishment Time Series (NETS) database \cite{walls2013national}, using a published algorithm that classifies specific food establishments as FFRs \cite{auchincloss2012improving}. Only distances shorter than one mile were kept for this analysis. This distance was chosen on the basis of previous work that estimated that the distance at which FFRs cease to have an effect on childhood obesity is approximately one mile \cite{baek2016distributed}.  Finally, we calculated the great circle distance between all schools, to derive a dataset of schools so that there are never two schools within one-mile of one another, in order to satisfy independence assumptions used in the analysis. 
\par
 
\par 
\subsection{Preliminary analysis}
\label{sec:prelim}
The dataset is comprised of 420,095 children who attended 1,228 high-schools. Across all high schools, 40\% of the 9th graders were observed to be obese. Of the high-schools, 782 had at least one FFR within one mile and 446 had zero.  Although the second stage analysis for the health outcome includes \emph{all} schools in the dataset, regardless of whether they have FFRs or not within a mile, the first stage analysis that derives clusters of school with similar spatial distribution of surrounding FFR  excludes the 446 schools that do not have any FFRs within one mile of their location. \\

Descriptive statistics of the schools are presented in Table \ref{tab:CA_descriptive}, for the entire dataset and for the two subsets of schools without FFRs or with at least one FFR within a mile.  As the Table shows, aside from having at least one FFR, schools included in the first stage analysis are generally more likely to be located in urban areas (46$\%$) compared to schools not included (27$\%$).   
Schools included in the first stage analysis varied both in terms of the number of nearby FFRs and in terms of their spatial distribution, both important aspects of BEF exposure. Among these schools, 45\% had 1 to 4 FFRs within a 1-mile buffer while the rest of the schools had at least 5; additionally the median (Q1-Q3) distance to the first FFR was 0.4 (0.3-0.6) miles . 
\begin{table}[H]
    \centering
\input{tables/descriptivetable}
    \caption{Descriptive Statistics for children and schools in the analytic dataset.   Summary statistics for categorical variables are the percentage of data in the column. IQR = Inter-quartile range.
    $\star$  17 schools have missing data on this variable information.}
    \label{tab:CA_descriptive}
\end{table}


A richer understanding of the exposure of schoolchildren to FFRs can be gleaned by examining the empirical cumulative distribution function (ECDF) of the distances between each school and its neighboring FFRs.  The ECDFs for four schools are shown in the top panels of Figure \ref{fig:composite_distance}. These two panels illustrate how traditional measures of built environment exposure, using simple counts or distance to the closest FFR, may fail to incorporate meaningful aspects of spatial exposure.
\begin{figure}[H]
    \centering
    \caption{panel A: Sample of schools with 10 Fast Food Restaurants (FFRs) within a 1 mile radius. Panel B: Sample of schools that have the same distance to closest FFR. Panel C: Sample of 100 schools distance to FFR 95\% distribution line ranges sorted by median distance to FFR. }
    \includegraphics[width = \textwidth]{figures/composite_distance_descriptive.png}
    \label{fig:composite_distance}
\end{figure}
Specifically, Figure \ref{fig:composite_distance}A illustrates how schools that may have a similar number of FFRs within a given distance may be characterized by a dramatically different spatial distributions of the surrounding FFRs. Likewise, Figure \ref{fig:composite_distance}B illustrates that while certain schools may have similar distances to the nearest FFR, the spatial distribution and the total number of nearby FFRs might be completely different. Characterizing exposure to FFRs on the basis of these traditional measures and clustering schools based only on how similar these two exposure metrics are across schools could miss meaningfully important aspects of spatial exposure, and consequently not fully capture the effect of exposure to unhealthy food on health. Panel C of Figure \ref{fig:composite_distance} illustrates the distribution of school-FFR distances for 100 randomly selected high schools, including the aforementioned four illustrative schools, further demonstrating the wide variability in exposure to FFRs in our dataset.  In order to accommodate the limitations in capturing exposure to FFRs discussed above, our modeling approach considers \emph{all} the distances from each school to its nearby FFRs, modeling this set of distances as a realization of a 1-dimensional point pattern whose school-specific intensity function is estimated non-parametrically. 
%Our model framework in the next section  will outline our approach supporting these two goals. 

==> Paper_Sections/Discussion.tex <==
In this work we have presented a two-stage modeling strategy that aims to provide epidemiological and social science investigators with a tool that permits them to both identify links between exposure to specific features of the built environment and health outcomes as well as identify those subjects at greatest risk of negative health outcomes.   In the first stage, our goal is to identify major patterns in the spatial distribution of FFRs around a school and group schools together based on their surrounding food environment. The second stage links the spatial distribution of FFRs around schools to the likelihood that children in the schools are obese. This work can be easily adapted to answer questions involving other point-referenced amenities in the built environment and other outcomes, for example, availability of parks and measures of physical activity\cite{evenson2016park} or depression \cite{bojorquez2018urban}, or availability of social engagement destinations and cognition, among others\cite{besser2018neighborhood}.
\par Our work breaks with previous approaches to address these questions in several ways. First, our clustering model differs from other parametric clustering models used in built environment research in that no constraints are imposed on the number of clusters. In addition to identifying the number of clusters, our model estimates the cluster specific densities non-parametrically, thanks to the use of the NDP prior on the density function representing the distances from a given school at which we expect to find FFRs.  This modeling strategy allowed us to identify clusters of high schools in California that have a high number of FFRs in their immediate environment relative to their peers, and those that have FFRs farther way. Additionally, through our proposed second-stage health outcome models, we showed how to incorporate information on the spatial distribution of point-pattern amenities into a health outcomes model, by using either a decision-theoretic framework or the posterior co-clustering probability matrix. These approaches identified that, independent of the quantity of FFRs within a mile of California high schools, children attending schools with FFRs further away had lower obesity risk. 

\par The second stage models have different advantages, disadvantages and ways of accounting for clustering assignment. Specifically, the CGLM has the potential to suffer from selection bias due to controlling uncertainty in cluster assignment by using only the subjects with highest certainty in their class assignment.  In our analysis, although the schools with higher uncertainty tended to have fewer outlets nearby, the excluded schools did not differ in terms of the outcome, thus minimizing selection bias concern upon conditioning by the number of FFRs in the second stage.  Users of the CGLM should keep in mind this potential for selection based on the outcome, in which case inverse probability of selection into the second stage could be used.  The BKMR uses all subjects, and handles cluster assignment uncertainty by using the co-clustering probability matrix -- essentially an average of cluster assignments between subjects. However, in reporting and discussing the results, we utilized the cluster mode assignment to help visualize/interpret the BKMR's rich set of output. We emphasize that, while the two-stage approach proposed here does not propagate uncertainty in cluster assignment in a standard fashion, this strategy still offers a number of benefits. For example, defining the exposure clusters independent of the outcome ensures a greater level of interpretability and conforms to substantive understanding of such clusters \cite{nylund2019prediction}. Furthermore, it offers a greater level of applicability, as clusters estimated in this fashion can be used for more than one analysis.

 Nevertheless , pursuing a method that more comprehensively propagates the uncertainty associated with cluster assignment through the health outcome analysis may be desirable. While both the BKMR and CGLM attempt to accommodate the uncertainty in cluster assignment through either restricting the analysis or averaging cluster assignment, neither fully estimates or propagates the uncertainty in the information (either single set of cluster labels or co-clustering probability matrix) through the health outcome model. One possible solution would be to develop a method that allows for joint estimation of both the cluster specific densities as well as the cluster associated higher outcome risk.  Our current method is unable to easily embrace such a joint modeling approach due to to both label switching and the varying the number of assigned clusters across the MCMC iterations, yielding identifiability problems for the outcome models \cite{gelman2013bayesian}. This makes the goal of joint estimation more difficult and a promising subject of future work. One possible solution would be to incorporate the health outcome at the level at which the cluster is constructed. Adapting the Logistic Stick Breaking Process \cite{ren2011logistic} for example, could facilitate this goal.  
 
 Further extensions of the work presented should incorporate the spatial distribution of more than one BEF amenity. The built environment consists of many amenities beyond FFRs that could be co-located with FFRs, or have different spatial distributions leading to different 'mixtures' of amenities. Extending our model to higher dimensions could allow investigators to characterize joint exposure to multiple amenities and identify their corresponding relationship with health outcomes. 
 \par 
 textcolor{blue}{revise this part of the text according to out conversation during Thursday's meeting - 08/13/2020}
 Finally, we acknowledge that there has been theoretical work showing that the DP cannot consistently estimate the number of clusters when the concentration parameter is fixed \cite{miller2013simple,miller2014inconsistency}. The same authors suppose a similar result holds in the more general case, though there is as yet no proof \cite{miller2018mixture}. While agnostic about this potential inconsistency, we remain optimistic that both the prior and likelihood can be used to appropriately penalize and inform the number of clusters, through the concentration parameter, resulting in model fit that is at least practically relevant, if not consistent. As \cite{gelman2013bayesian} writes, ``It may seem counter intuitive that the data can inform strongly about the number of clusters through the hyper parameter $\alpha$ [concentration parameter] given that maximum likelihood estimation leads to over fitting, with more clusters resulting in a higher maximized likelihood. However, the Bayesian approach favors clustering and values of $\alpha$ that result in a high marginal likelihood. If individuals are allocated to many different clusters, the effective number of parameters in the likelihood is increased, and we then integrate across a larger space in calculating the marginal likelihood.'' This sentiment has held up in our simulations, whereby including the concentration parameter $\alpha$ in our model has led to correct estimates of the number of clusters.

 \textcolor{red}{What else should be said here? Address limitations common to non-parametric methods?} \textcolor{blue}{I think there should be discussion of the fact that even if our modeling strategy is attempting to incorporate clustering assignment uncertainty, it still does not do that completely. And so the discussion should include some text as for how to propagate cluster assignment uncertainty in oNE JOINT MODEL rather than through a two-stage approach as we have done. I think you have to discuss the problems with cluster identification in DP and NDP. I think that what  you have now regarding potential extensions/future work, should be at the end of this section. But this section needs to be expanded.}

==> Paper_Sections/Introduction.tex <==
\large

The dramatic increase in child obesity is one of the most pressing public health issues of the 21st century \cite{world2012population}. The potential causes of lack of energy balance that result in child obesity have been widely studied, and the need for population-level interventions, beyond individual-level treatments has been strongly emphasized by the research community and policy makers alike \cite{IOM}. Place-based interventions are one realm of population level approaches that seek to modify neighborhood environments in ways that can support residents' health promoting behaviors. Within this type of approaches, changes to the distribution of health-supportive (or detrimental) amenities within neighborhood environments have emerged as a possibility, given that the built environment--the human made space in which humans live, work and recreate on a day-to-day basis \cite{roof2008public}--constrains everyday health-relevant choices. 

In particular, the potential contribution of the food environment near schools (e.g., fast food restaurant availability) to child obesity has been studied extensively  \cite{currie2010effect,davis2009proximity,sanchez2012differential,baek2016distributed}, given that children spend large proportions of their waking hours and consume a large proportion of their food within and near the school environment.  While the body of evidence supports these connections broadly, different approaches to conceptualize exposure make it challenging to more fully understand the health effects of environmental exposures, as well as identify where interventions may be especially needed. In order to assist policy makers with these challenges, methods need to be developed that both (i) identify different spatial patterns of exposure and (ii) link these patterns to health outcomes quantitatively. Exposure patterns, compared to continuous exposure measures, may make it more straightforward to identify places in higher need of interventions.
\par 
Previous work in environmental epidemiology has approached these problems by first clustering some measure of built environment features (BEFs), e.g. the number of fast food restaurants (FFR) or nearby park accessibility, and then incorporating cluster assignments as a categorical predictor into a second stage regression model. For example, \cite{wall2012patterns} used a spatial latent class analysis (LCA) \cite{wall2009spatial} to cluster multivariate measures of the built environment, including the density of food outlets within 1 mile of the subjects residential location, and subsequently estimated the association between cluster membership and adolescent obesity. Like \cite{wall2012patterns}'s analysis, it is common\cite{an2012school,howard2011proximity} to use a simple density or count of BEFs within some pre-specified buffer (e.g. 1 mile) as an exposure measure. However, this assumes that the effect of each BEF is identical across the buffer, an assumption that is not empirically supported \cite{baek2016distributed,fotheringham1991modifiable}\textcolor{blue}{not completely sure about this statement. I think we need to be careful about spatially-varying covariates and spatially-varying coefficients, which it seems to me this sentence is referring to}. Consequently, the clusters identified ignore the spatial distribution of amenities within the buffer. This spatial distribution is relevant from a mechanistic perspective because BEFs closer to schools are easier to access, as well as policy relevant since the distribution could inform built environment interventions such as zoning laws to curtail exposure.  Finally, plugging in an estimate of cluster membership as a predictor in a health outcome model does not account for the uncertainty in the estimated cluster assignment label, leading to potentially incorrect inference of the associated health effect.

Motivated by the need to better understand the association between exposures to FFRs near schools and child obesity, this paper has two complementary goals. First, we aim to develop a clustering procedure that provides interpretable groupings of BEF exposure while taking into account the spatial distribution of BEFs.  For this goal, we work with the geographical coordinates of BEFs and schools, modeling the set of distances of each school to its nearby BEFs as a realization of a 1-dimensional point pattern with a school-specific intensity function. Clusters of schools are formed by clustering the intensity functions of these point patterns using a Nested Dirichlet Process (NDP). Working with point-level data and using the actual distances between schools and BEFs, rather than aggregating the data at the areal-unit level, allows us to maintain the level of granularity needed to investigate the effect of the spatial distribution of BEFs around schools on children's obesity. In particular, our approach to deriving the schools' cluster assignments is based on the distribution of distances of schools and their surrounding FFRs, but not the quantity of FFRs. This clustering approach enables us to separate the contribution to obesity associated with the number of FFRs near schools that is independent from their relative proximity to the school in the health outcome regression model, thereby providing new insights compared to prior work investigating the relationship between FFRs availability and obesity. Second, we show two ways to use the output from the NDP clustering model to address cluster assignment uncertainty when using clusters as predictors in a regression that evaluates the association between FFR exposure near schools and obesity risk of students in those schools.   
 \par 

As a statistical genre, clustering methods vary widely, from the model-based finite mixture models (FMM)\cite{diebolt1994estimation} and previously mentioned LCA \cite{wall2009spatial}, to the more algorithmic k-means style methods \cite{hartigan1975clustering,friedman2001elements}. Each of these have varying strengths and weaknesses according to the problem at hand. Notably, FMMs, K-means and LCA share the important assumption of pre-specifying the number of clusters that should be found in the data. LCA and K-means also make parametric assumptions about the relevant distribution or metric, respectively, that should define the clusters. In our pursuit of examining the contribution of both the spatial distribution and quantity of FFRs around schools on obesity without strong parametric assumptions or pre-specification of the number of clusters we employ a NDP approach. We use the NDP to flexibly cluster schools according to the  spatial distribution of BEFs around them, which we assume is regulated for each school by the intensity function of an Inhomogenous Poisson Process (IPP). The NDP allows us to estimate these functions without enforcing any strong parametric constraints on the shape of the intensity function or the number of clusters. Additionally, in accordance with our conceptual objective (i), the NDP provides cluster assignment labels  which can be processed and used in a second-stage regression analysis to estimate associations between the BEF's spatial distribution and a health outcome of interest.  \textcolor{blue}{Here add text with reference to the paper by Kottas et al.} 

The need to accommodate uncertainty in estimated exposures (in this case cluster assignment) has been the topic of several papers \cite{chiang2017hierarchical,graziani2015bayesian,wall2012patterns,wade2018bayesian}. Here, we explore two approaches to using the output of our clustering model in a second-stage analysis as a way to deal with the challenges of making cluster assignments; namely the NDP yields a varying number of cluster assignments in the posterior samples. One approach relies on using a conservative ``consensus of cluster assignments'' as determined from cluster-specific uncertainty bounds\cite{wade2018bayesian}. The second approach avoids the use of a single cluster assignment by using each school's vector of co-clustering probabilities with other schools as a measure of multivariate exposures, inserting the vector as a predictor  into a health outcome model through a Bayesian kernel machine (BKMR) regression \cite{bobb2015bayesian} approach \cite{valeri2017joint,coker2018association,wang2018associations}. This latter approach is an innovation in terms of expanding the applications of BKMR, as well as a way to utilize a clustering model's output. 
\par 
The layout of the paper is as follows: Section 2 discusses the data sources used in our analysis of child obesity in relation to FFR near their schools, namely data on children's' obesity status and school characteristics obtained from the California Department of Education, and food outlet locations from the National Establishment Time Series (NETS) database. The section includes discussion of some nuances involved in handling this and similar data for our proposed statistical methodology, as well as some preliminary data analysis. Section 3 describes the modeling approach that we propose for clustering schools with respect to the spatial distribution of FFRs around the school and the two modeling frameworks for the second stage health analysis.  Section 4 contains the results from fitting our models to the California data. We finish with a discussion of the contribution our work makes to the built environment literature, limitations of our approach and possible methodological extensions.


\textcolor{red}{In case we need/want it, the .tex file has a paragraph (hidden from the pdf) that reviews the applications of NDP more broadly.} \textcolor{blue}{I would put that paragraph before the paragraph that discusses the second-stage analysis, e.g. the health outcome model, however I think that I would like to rewrite it. I think we do have to make a reference to the paper by Kottas et al. However the argument that our difference is that we want to account for variability between and within school to me is not the main difference between our model and the model of Kottas. I bet his models also account for that... So, I think we need something a little bit more specific.}
\begin{comment}
\par

There is a large literature devoted to applications of IPP for modeling spatial point processes and non-parametric estimation of the intensity function. While our work is inspired by the reading of \cite{xiao2015modeling,taddy2012mixture}, the use of a Dirichlet Process (DP) to flexibly estimate the intensity function of an IPP was first developed by \cite{kottas2007bayesian,kottas2006dirichlet} in applications related to extreme value analysis. However this approach has found traction in areas as diverse as neurology \cite{ihler2007learning} and immunology \cite{ji2009spatial}. The fundamental difference between those papers and our approach, is that we are not as concerned with introducing dependency in the DP for the sake of accommodating spatio-temporal dependence between observations, but rather to account for the variability between and within the school intensity functions. Consequently we looked to the NDP whose development was motivated by multilevel clustering of probability distributions in nested data settings. While the NDP has previously found applications in clustering the error distributions in hospital quality of care \cite{rodriguez2008nested}  and neurological fiber connections \cite{zhang2019nonparametric} data, this is the first application to our knowledge of using the NDP in the context of estimating spatial IPPs. \textcolor{blue}{Need to work on this}
\end{comment}
\par 

==> Paper_Sections/Model.tex <==
As mentioned in Section~\ref{sec:Intro}, our analysis of the effect of exposure to FFRs on obesity is based on a two-stage approach: (i) a first model that characterizes the main patterns of school-level exposure to FFR, by deriving characteristic profiles of the spatial distribution of FFRs near schools; (ii) a second model that uses the output from stage 1 in a regression model that examines the association between patterns of exposure with child obesity. In the following sections we provide details of each of these modeling strategies, including specific aspects of our models' implementations and estimation.


\subsection{Clustering model}
\label{sec:mod_cluster}
Let $r_{ij}$ be the distance between the $i$th school $(i=1,...,N)$ and the $j$th nearby FFR $(j=1,...,n_i)$: each $r_{ij}$ belongs to the interval $(0,R) \subset \mathbb{R}$, with maximum distance $R$ chosen on substantive grounds.  For each school $i$, we model the random subset $\mathcal{D}_i = \{r_{ij} ;j =1,...,n_i\} \subset (0,R)$ as a realization from a one-dimensional Inhomogeneous Poisson Process (IPP) with intensity function $\lambda_i(r), r\in (0,R)$. We further decompose the intensity function $\lambda_i(r)$ as $\lambda_i(r)=\gamma_i f_i(r)$ with $\gamma_i$ representing the expected number of FFRs within radius $R$ from school $i$ and $f_i(r)$ denoting a normalized density. Thus, the $i$th school's contribution to the likelihood is: 
\begin{displaymath}
p\left( \mathcal{D}_i | \gamma_i,f_i(r)  \right) \propto  \gamma_i^{n_i}\exp\{-\gamma_i\} \prod_{j=1}^{n_i} f_i(r_{ij}). \label{eqn:mod_llhood} \tag{1}    
\end{displaymath}
Assuming independence between schools, the full likelihood is obtained by taking the product over the $N$ schools likelihood contributions. In (\ref{eqn:mod_llhood}) we note that the  likelihood is separated into a component that handles the random number, $n_i$, of FFRs for each school $i$, and a component that, given $n_i$ FFRs surrounding school $i$, evaluates the density at each of the $n_i$ distances. For our purposes, $\gamma_i,i=1,...,N$ are considered nuisance parameters that do not affect the estimation or interpretation of the $f_i(r)$ beyond what has been previously discussed, nor the second stage outcome model. In the health outcome model we use the observed $n_i$'s directly as a predictor, instead of its expected value $\gamma_i$, in accordance with our aim to differentiate between the separate effects of the observed FFR quantity and FFRs' spatial distribution on childhood obesity.

\par Our goal is to simultaneously model and cluster the FFR spatial density functions $f_i(r)$, $i=1,\ldots,N$, in a non-parametric fashion.
The non-parametric estimation of a single $f_i(r)$ could be accomplished by using a Dirichlet Process (DP) mixture model \cite{gelman2013bayesian}. However, in order to fulfill our goal of non-parametrically estimating and clustering the $f_i(r)$'s themselves, we use a NDP modeling approach.  The NDP enables us to achieve both of these objectives through the use of two DP's simultaneously. Specifically, we express each $f_i(r)$ as: 
\begin{align*}
    f_i(r) &= \int \mathcal{K}(r|\bm{\theta})dG_i(\bm{\theta}) \label{eqn:mod_ndp1} \tag{2}\\
    G_i &\stackrel{iid}{\sim} Q\\
    Q &\sim DP(\alpha,DP(\rho,G_0)),
\end{align*}
where, $\mathcal{K}(r|\bm{\theta})$ is a mixing kernel with  parameter vector $\bm{\theta}$, and the distribution $G_i$ is drawn from the random distribution $Q$ on which we place a NDP prior. In (2), $DP(\rho,G_0)$ denotes a DP with concentration parameter, $\rho>0$, and parametric base measure, $G_0$. The base measure $G_0$ is the distribution around which the DP is centered and the concentration parameter, $\beta$, reflects the variability around that base measure.
\par It is through the $G_i$'s that the $f_i(r)$'s are clustered as can be seen from the stick breaking construction representation of the NDP: $Q = \sum_{k=1}^{\infty} \pi_k^*\delta_{G_k^*}(\cdot)$. In this representation, $\pi_k^*$ represents the probability that a school is assigned to the $k$-th mixing measure, $G^{\star}_k$, $\delta_{\cdot}(\cdot)$ is the Dirac delta and $G_k^*= \sum_{l=1}^{\infty} w_{lk}^{*} \delta_{\bm{\theta}^{\star}_{lk}}(\cdot)$ is itself composed of weights, $w_{lk}^*$ and associated atoms $\bm{\theta}_{lk}^*$. This hierarchy of distributions, weights and atoms provides a framework that flexibly identifies clusters of schools, and also flexibly estimates the intensity function representing the spatial distribution of FFRs surrounding schools for each cluster. 

Combining it altogether, the hierarchical formulation of our model is:
\begin{align*}
\{r_{ij} ;j =1,...,n_i\} &\stackrel{ind}{\sim} IPP(\lambda_i(r)), \quad i = 1,\ldots,N \label{eqn:mod_ndp2}\tag{3}\\
%\{r_{ij}\}_{j=1}^{n_i} &\sim IPP(\lambda_i(r)), \quad i = 1,...,N\\
\lambda_i(r) & = \gamma_i f_i(r)  \\
    f_i(r) &= \int \mathcal{K}(r|\bm{\theta}) dG_i(\bm{\theta})\\
    G_i & \stackrel{iid}{\sim} Q\\
    Q & \sim DP(\alpha, DP(\beta,G_0)) 
\end{align*}




\par
In our analysis of FFR exposure around California public high schools we transform the school-FFR distances from $(0,R) \to \mathbb{R}$ using a probit function to create the modified distances $r'_{ij}=\Phi^{-1}(r_{ij}/R)$. We make this transformation in order to use a normal mixing kernel and corresponding normal-inverse-chi square base measure, $G_0 = N(0,\sigma)\times\text{Inv}-\chi^2(1,1)$, in order to facilitate computation. Similarly, we place informative Gamma priors, on the concentration parameters, $\alpha,\beta \sim \text{Gamma}(10,10)$, to encode our \textit{a priori} belief that there should be a small number of clusters, in line with similar work \cite{ishwaran2001gibbs,gelman2013bayesian,rodriguez2008nested}. 





\subsection{Health Outcomes Model}
\label{sec:mod_outcomes}
In the second stage of the analysis, we examine how spatial distributions of FFRs around a school, more specifically, patterns of spatial distributions of FFRs around a school, are associated with obesity of children in the school. For this, we use results from the clustering model as input in to a regression model where child obesity is the outcome. 
%There are some difficulties in doing this.  First, since the number of clusters is not fixed, each posterior sample of cluster assignments may have a different number clusters assigned. Consequently, creative solutions are required to handle the NDP output since straightforward ``plug-in'' methods do not yield sensible answers. \textcolor{red}{In addition, (insert text here about sources of uncertainty). also, we need to re-work the text below after the group discussion on this} 

 \par The simplest way to do this would to be to assign a cluster label to each school and use it as a covariate in the health outcome regression. However, proceeding in this fashion would not account for the uncertainty in the cluster assignment and would not exploit all the information in the posterior samples that are generated while fitting the clustering model of Section \ref{sec:mod_cluster}. To address these issues, we propose two alternative approaches.
 
 \par \textbf{Consensus generalized linear model (CGLM)}. The first approach \emph{controls} uncertainty in the cluster labels by using in the health outcome model only the schools for which the cluster label is known with greater relative certainty, as follows.  First, we derive cluster assignment labels for each school using the posterior samples and a loss function in a decision theoretic framework\cite{wade2018bayesian}. Specifically, we use the variation of information (VI) loss function to determine the optimal cluster configuration, which simultaneously identifies both  the number of clusters and cluster labels for the schools. This approach finds the posterior sample that produces the minimal loss, and uses the number of clusters and cluster assignments in that sample to assign labels to schools-- thus deriving, essentially, a 'point estimate' for the discreet/categorical cluster assignment. We refer to this point estimate as the `mode' cluster label. \\
 
 Second, we identify schools with low uncertainty in the cluster label. In addition to the mode cluster configuration, the method \cite{wade2018bayesian} also produces 95\% uncertainty bounds for both the number of clusters and for the cluster labels for each school, yielding three additional cluster configurations (for a total of four including the mode). Compared to typical ``upper'' and ``lower'' bounds, the method provides three bounds according to the combination of loss metric value and the number of clusters, the latter of which can vary from one configuration to another.   Since, as noted earlier, employing the cluster labels from the single point estimate as a predictor in the health outcome model would ignore the uncertainty associated with the cluster assignment label, our goal here is to take into account all four cluster configurations to control or reduce the uncertainty. One possibility is to use each of the four assignments in separate health outcome regression models, and subsequently fuse together their results. However, fusing those four models may entail fusing models with potentially a different number of clusters. Thus, rather than using each of the four alternative cluster labels in the health outcome models, we restrict the health outcome analysis to the set of schools that are assigned to the same cluster across the four different cluster assignments. Note that this is only possible when clusters are well identified and posterior samples do not exhibit label-switching across iterations \cite{gelman2013bayesian}, or a post-processing step that adjusts for label switching has been run \cite{rodriguez2014label,stephens2000dealing,panagiotis}. These conditions ensure that cluster labels are consistent across configurations and, consequently, taking the intersection has a consistent meaning. \\  
 
In summary, the CGLM approach addresses the uncertainty in the cluster label assignment by taking the intersection of the four cluster labels to arrive at a more conservative (less uncertain) estimate of the schools' cluster assignment. This reduction of uncertainty in cluster assignment comes at the cost of sample size, as schools will be included or excluded from the health regression model according to whether they fall within said intersection or not. Despite this loss of sample size, the key advantages of this approach are that this enables a straightforward analysis, as the intersection of the four cluster configurations yields a single cluster assignment for each school that can be used as a categorical covariate in the health outcome model, and the cluster assignment is more precise than the single 'point estimate' label in the entire sample.\\ 
 
To define the CGLM outcome model and enable us to distinguish the association between the quantity of FFRs and obesity from that of the FFRs' spatial distribution, we bring back into consideration the schools that had zero FFRs within 1 mile. Let $C_{i,k} = I(\text{ith school belongs to cluster k})$, $k=1,...,K$, denote the cluster to which the $i$-th school is assigned ($K=6$ in our analysis). In addition, define $Q_{i,m}, m=0,...,M$ a set of indicator variables that treat the number of FFRs as a categorical variable. In particular $Q_{i,0}=I(n_i=0)$, with the other categories being $ n_i=2;n_i=3; n_i=4; n_i \in \{5, 6, 7\},$ and $n_i>7$.  This categorical representation is used given the distribution of FFRs and the lack of linearity in the association between FFR quantity and the odds of obesity. We note that the cluster indicators are only available for schools with $n_i>0$, and that the schools included in this model are those with $n_i>0$ that are determined by the consensus approach discussed above to have a cluster label with relatively higher certainty, along with schools with 0 FFRs. This set of schools is denoted as $\mathbb{D}_{CGLM}$. \\

The GCLM model linking obesity in schoolchildren to exposure to FFRs and other school neighborhood characteristics is thus: 
 \begin{align*}
\text{logit}(\pi_{i'}) = \left\{ \sum_{m=0}^{M}Q_{i',m}\zeta_{m}\right\} + I(n_{i'}>0)\left\{ \sum_{k=1}^{K} C_{i',k}\xi_k \right\} + \bm{Z}_{i'}^{T} \bm{\beta} \qquad i' \in \mathbb{D}_{CGLM} \label{eqn:outcomes_cglm} \tag{5}
 \end{align*}  
 In (\ref{5}) $\pi_{i'}$ denotes the proportion of obese 9th grade students at the $i'$th high school, $\zeta_{m}$ and $\xi_k$ are quantity- and cluster-specific intercepts, respectively (i.e., cell means coding) and  $\bm{Z}_i$ is a vector of school characteristics without an intercept term.  
 
 


\par  \textbf{Bayesian Kernel Machine Regression (BMKR)}.  \textcolor{red}{Veronica brought up a lot of concepts that we need to highlight. I've edited  for length and to streamline. The full text is still available in the other version in case I butchered the text! - Brisa.} In the second approach, we move away from using a categorical predictor in the health outcome model, and instead use BKMR, as explained below, to input the probabilities that any pair of schools belong to the same cluster into the health outcome model. This has several advantages compared to approaches that use a single set of cluster labels for schools (e.g., the mode) in the heath outcome model. When a categorical predictor,  denoting discrete groups of schools' FFR spatial profiles, is used in the health outcome model, we estimate the effect of each of these spatial profiles by borrowing information only from the schools within the same clusters. Hence, when we estimate health effects in this fashion,  we are only borrowing information from a limited number of schools, those that belong to the same disjoint subsets of schools, i.e., clusters. Moreover, as described above in the CGLM, additional steps are needed to account for cluster assignment uncertainty. In contrast to the CGLM specifically, which controls uncertainty by restricting the sample, the BKMR utilizes all the schools in the NDP.
 
 The BKMR approach proceeds as follows. First, to each school $i$, $i=1,\ldots,N$, in the clustering sample, we associate the $N$-dimensional row-vector $\mathbf{P}_i$, $i$-th row of the co-clustering probability matrix $\mathbf{P}$. This matrix is constructed by averaging, for each $i$, the indicators $I(\text{school}~i~\text{and}~j~\text{are in the same cluster})$, for $j\neq i$ across the posterior samples, with the $i$-th element of $\mathbf{P}_i$ set equal to 1 by convention. By using the $N$-dimensional vector $\mathbf{P}_i$ as a predictor in the health outcome model, we allow all schools, including those that  would not be assigned to the same cluster as school $i$ when using a loss function or other criteria, to contribute to the estimation of the effect of the spatial distribution of FFRs surrounding the school on its schoolchildren's odds of obesity.  In other words, in this approach we remove the hard boundaries that separate schools into disjoint subsets, and enable sharing of information about schools' FFR-spatial profiles across all schools, albeit the contribution of schools with more (compared to less) similar profiles is given higher weight. 

\textcolor{red}{from Brisa: I removed the "we are now confronted with the problem of at least as many predictors as observations".... which is a problem of our own making. However, I did keep the references to environmental epi towards the end of the paragraph.}
Second, rather than linking the log-odds of obesity at school $i$ to the $N$-dimensional row-vector $\mathbf{P}_i$, directly, in the logistic regression for obesity, we include as a \emph{predictor} the scalar $h(\mathbf{P}_i)$ for school $i$. Since schools that have large probabilities of being co-clustered are likely to have similar $N$-dimensional row-vectors, while schools that are not very likely to be co-clustered are associated with more dissimilar $N$-dimensional row vectors, we model the $N$ random terms  $h(\mathbf{P}_i)$, $i=1,\ldots,N$ jointly. Specifically, we model $\left( h(\mathbf{P}_1), \ldots,h(\mathbf{P}_N) \right)$ as a finite-dimensional realization of a Gaussian process with mean $\bm{0}$ and Gaussian covariance function $\kappa(\cdot, \cdot; \phi, \sigma^2)$.  The covariance function $\kappa(\cdot, \cdot; \phi, \sigma^2)$ is evaluated using as distance between any two $N$-dimensional row-vectors $\mathbf{P}_i$ and $\mathbf{P}_j$ the Euclidean distance, whereas the two parameters $\phi$ and $\sigma^2$ encode, respectively, the range of the correlation, e.g. the distance at which the correlation between any two $N$-dimensional random vectors is essentially negligible, and the marginal variance of each $h(\mathbf{P}_i)$. This approach borrows from the environmental epidemiological literature where researchers are often confronted with the issue of having multiple, potentially correlated, high-dimensional exposures.\\

As with the CGLM, we incorporate into the outcome model all observations with 0 FFRs within the mile, and use the indicators for quantity of FFRs nearby, $Q_{i,m}$, to distinguish the effect on obesity associated with the quantity of FFRs from their spatial distribution. Altogether, the second health outcome model is:
\begin{align*}
    \text{logit}(\pi_{i'}) &= 
    Q_{i',0}\zeta_{0}+ I(n_{i'}>0)\left\{\tilde{\alpha}  + h(\bm{P}_{i}) +  \sum_{m=0}^{M}Q_{i',m}\zeta_{m} \right\} + \bm{Z}_{i'}^{T} \bm{\beta}  \quad i' \in \mathbb{D}_{BKMR}  \label{eqn:outcomes_bkmr} \tag{6}\\
    h(\cdot) &\sim \mathcal{GP}(\bm{0},\kappa(\cdot,\cdot|\phi,\sigma^2)). 
\end{align*}
 In (\ref{eqn:outcomes_bkmr}), $\mathbb{D}_{BKMR}$ is the index set for schools used to fit the BKMR model, i.e., schools with zero FFRs in addition to the full set of $N$ schools in the first stage. Additionally, $\tilde{\alpha}$ denotes the intercept for schools with at least one FFR, and $h(\bm{P}_{i'})$, $i' \in \mathbb{D}_{BKMR}$, indicates a school-specific random intercept. The other components of the model in (\ref{eqn:outcomes_bkmr}) - $\bm{\beta},\bm{Z}_{i'}$ - have the same definition and interpretation as before. 
 

 
 \par In the CGLM and BKMR models, $\bm{\beta}$, $\zeta_m$,$m=1,...,M$ and $\xi_k$, $k=1,...K$ are given flat improper priors, while in the BKMR, $\phi$ and $\sigma^2$ are each given informative folded Normal$(1,3)$ priors to accommodate known identifiability issues \cite{zhang2004inconsistent}. These informative priors were chosen after initial runs with a uniform prior on a larger domain showed samples in the $(0,1)$ interval.

\subsection{Estimation}
\label{sec:Estimation}

As both the clustering model and the two health outcome models that we have proposed in Section \ref{sec:mod_outcomes} are specified within a Bayesian framework, inference on all models parameters is obtained through the posterior distribution, which we approximate using Markov chain Monte Carlo (MCMC) algorithms. For the NDP clustering model we use the blocked Gibbs sampler as described in \cite{rodriguez2008nested}, truncating the summations for the inner and outer DPs using $L=30$ and $K=35$, respectively - a choice based on logic similar to that discussed in \cite{rodriguez2008nested}. This model fitting routine is implemented within our  \texttt{bendr} \cite{bendr} \texttt{R} package.  The health outcome models are fit using the Hamiltonian Monte Carlo variant sampler implemented in \texttt{stan} \cite{carpenter2016stan} via \texttt{rstan} (BKMR) \cite{rstan} and \texttt{rstanarm} (CGLM) \cite{rstanarm}. All model fitting was performed within \texttt{R} (v.3.6.1) \cite{Rlanguage} on a Linux Centos 7 operating system with 2x 3.0 GHz Intel Xeon Gold 6154 processors.
\par For the NDP model, 250,000 samples were drawn from the posterior distribution, with 240,000 iterations discarded for burnin-in and the last 10,000 iterations thinned by 3 to reduce auto-correlation for a total of 3,333 posterior samples used for inference. The length of the burn-in period and thinning were determined by inspecting trace plots for various model parameters and by computing Raftery's diagnostic statistic\cite{raftery1995number}. 
For both health outcomes models, we ran 4 independent chains, using different initial values and each ran for 2000 iterations. For each chain, we kept 1000 samples after burn-in, for a total of 4000 posterior samples that we employed for posterior inference. Convergence was assessed via split $\hat{R}$ \cite{gelman2013bayesian} and visual inspection of trace plots. 
\par In fitting both proposed health outcome models, we note that 17 schools previously included for analysis in the clustering model cannot be included in the health regression models as they are missing outcome information. However, as discussed in Section \ref{sec:mod_outcomes}, both logistic regressions for obesity include an additional 446 high schools with no FFRs within the 1 mile radius, which were not considered in the clustering model. Cluster labels that are included as predictors in the CGLM model were derived using the \texttt{mcclust.ext2} package \cite{mcclust} employed to estimate the posterior assignment credible bounds with VI as loss function as detailed in \cite{wade2018bayesian}. We take the intersection over the horizontal, upper and lower bounds as described in Section \ref{sec:mod_outcomes} to arrive at our cluster assignment predictors for the CGLM. \\

For the NDP, posterior medians, inter-quartile ranges (IQRs) and 95\% credible intervals are calculated for the intensity function parameters, $(\mu_{lk},\sigma^2_{lk})^*$, $\pi^*_k$ as well as the average probability of co-cluster membership $\bm{P}$ as described in Section \ref{sec:mod_outcomes}. The $f(r)$ were constructed over a fine grid of equally spaced values in $\mathbb{R}$ representing the distances of a BEF from a school, combining the $K$ clusters and $L$ within-cluster components at each distance. 
Since, for computational purposes, we transformed the school distances to BEF from the interval $(0,R)$ to $\mathbb{R}$, when inferring upon the actual densities $f(r), r\in (0,R)$, we back-transform them onto the $(0,R)$ domain using the inverse probit function,  rescaling them by an empirically calculated proportionality constant. 

\par In the health outcome models, posterior median and 95\% credible intervals are calculated for regression coefficients $\bm{\beta}$,cluster effects $\xi_k, k=1,...,6$, and $\bm{h}(\bm{P}_i)$. Additionally, the effects of FFR quantity, as described in Section \ref{sec:prob_calc}, were also calculated.

\subsubsection{Non-Standard Probability Calculations}
\label{sec:prob_calc}

Given that schools with $n_i=0$ cannot be assigned a cluster for obvious reasons, the CGLM includes the non-standard interaction terms between quantity $n_{i'}>0$ and cluster assignment.  As in any model with interactions, describing the `main effect' of an exposure requires careful attention. In this case, the `main effect' of the quantity of FFRs depends on the cluster to which schools with $n_{i'}>0$ were assigned. For each category 
 $Q_{i',m}$ with $m>0$, we marginalize over the cluster assignment to define the probability  of obesity given category $Q_{i',m}$. \textcolor{blue}{make sure to correct all the following text to condition on $\mathbf{Z}_i=\mathbf{0}$, having defined what $\mathbf{Z}_i$ is and what is the reference class, e.g. what does $\mathbf{Z}_=\mathbf{0}$ means. Also remember that these are posterior distribution, we we should condition on the data.} That is the \emph{quantity effect}, holding $Z_i$ constant, is $P(\text{Obesity}|Q_m) = \sum_{k=1}^{K} p_k\text{inv-logit}(\zeta_m + \xi_k)$, where $p_k$ is the probability of a school being assigned to cluster $K$ in the $\mathbb{D}_{CGLM}$ dataset. Note that for $n_i=1$ , there is no corresponding effect, $\zeta_1$, as this is defined as the average cluster effect by the construction of the model in (\ref{eqn:outcomes_cglm}).
 \textcolor{blue}{Same comments here: (i) conditioning on the data, since this is a posterior distribution; (ii)also specify what $\mathbf{Z}_i$ is.}Similarly, for the BKMR we calculate the \textit{quantity effect} of FFR on schoolchild obesity, now averaging over the $h_i(\bm{P})$'s, using the following probability expression P(Obesity$|\zeta_m) =  \frac{1}{\mid \mathbb{D}_{BKMR} \mid} \sum_{i=1}^{\mid\mathbb{D}_{BKMR}\mid} \text{inv-logit}(\zeta_m + \hat{h}_i) $, where $\hat{h}_i$ is the posterior mean estimate.

==> Paper_Sections/Results.tex <==
We now discuss results from both the clustering model, that aims to identify major patterns in the spatial distribution of FFRs in a 1 mile radius ($R=1$) around schools, and the health outcomes models that relate the spatial distribution of FFRs to the odds of obesity in schoolchildren.

\subsection{Spatial Intensity Functions}

\par 
The clustering model estimates six clusters with high probability, with the estimates of the cluster-assignment probabilities, $\pi^*_k$, beyond the first six effectively negligible when rounding to the hundredths place. The median density estimates, representing the likelihood of finding an FFR at a given distance from a school, are presented in Figure \ref{fig:est_clusters}, along with the percent in each cluster. Note that these density estimates, estimated during model fitting on the real line are transformed back to the bounded interval $(0,R)$ miles for ease of interpretation.  As the figure shows, clusters are labeled according to their mode's proximity to the school, i.e. the cluster which estimates most FFRs to be located nearest to schools is labeled cluster 1, and so forth. A figure with the densities on the real line as estimated in the model along with 95\% credible intervals is shown in the Supplementary Material. 

%\begin{table}[H]
%\centering
%\input{tables/pi_table}
%\label{tab:probs}
%\end{table}


\begin{figure}[H]
    \centering
    \includegraphics[width = .9 \textwidth ]{figures/cluster_intensities_one+pcts.png}
    \caption{Median estimate of cluster density functions $f^{*}_k(r)$, $k=1,\ldots,6$, with the estimated percent of schools within each cluster, $\pi^*_k$. The IQR for the percent of schools in each cluster are, for clusters 1 to 6, respectively: 3, 2, 4, 5, 5, and 2$\%$}
    \label{fig:est_clusters}
\end{figure}

In order to visualize how distinctly the clustering model assigns schools into the six different clusters Figure \ref{fig:pairwiseplot} presents a heat map of the co-clustering probability matrix $\mathbf{P}$. Note that in the Figure, for the sake of visualization, school indices are arranged so that schools with similar co-clustering probabilities are next to one another, as implemented in the algorithm described in \cite{rodriguez2008nested}'s Supplementary Material. Examining the plot, we can clearly see the six clusters from left to right followed by the remaining schools which the model cannot cluster consistently.  

\begin{figure}[H]
    \centering
    \includegraphics[width =  .9\textwidth ]{figures/pairwiseplot.png}
    \caption{Heat map of co-clustering probabilities, that is, the probability that any two schools are assigned to the same cluster. The identity line may be interpreted as a school's probability of being clustered with itself. Although this probability is trivially equal to 1, for plotting purposes, in the figure this line is left equal to 0 to more clearly show the plot's line of symmetry.}
    \label{fig:pairwiseplot}
\end{figure}

Table 3 presents summary statistics for the characteristics of the schools included in the six clusters identified , including a tabulation of the categorical variable describing the number of FFRs within a 1-mile of each school. In the table, we also include the characteristics of schools for high schools that have no FFRs within one mile of their location: we label this cluster as ``Cluster 0''.
There is a weak association between a school's census tract median household income in Table  \ref{tab:cluster_table} \textcolor{blue}{This table has a weird numbering, like 4.1?!} and cluster membership. While Cluster 1's median census tract median income is \$55,200, Cluster 6's median census tract median income is \$67,400. However, this patterning does not include Cluster 0, which has a lower median census tract median income of \$53,800. A similar, though even weaker, pattern can be seen in the proportion of residents in the schools' census tracts with 16 or more years of education. Forty-two percent of schools in cluster 1 have  majority of white students populations, whereas 37 have predominately Latino students; for cluster 6, these percentages change to 48 and 16, respectively. Notably, all clusters contain schools across all urbanicity classification, and include schools with a varying number of FFRs. In other words, the mode cluster is not driven by quantity or broader context (urbanicity) of the schools. 

To assess whether the six identified clusters were geographically concentrated in one or more sub regions of California, and to investigate whether schools tended to co-cluster with nearby schools,  we produced spatial plots of the co-clustering probabilities for a given school. Figure \ref{fig:probmap} presents this plot for a school located in Southern California, identified in the map by a star symbol. As the figure shows, the schools that are more likely to be co-clustered with the selected school are not necessarily located nearby. Rather, as the first panel of the figure shows, most of the schools nearby the chosen school tend to have a probability smaller than 0.5 of being assigned to the same cluster.
\begin{landscape}
\begin{table}[H]
\centering 
\small
\input{tables/cluster_table}
\label{tab:cluster_table}
\caption{Cluster demographic descriptive summary. Summary statistics - percents, median and inter-quartile range (IQR) for categorical and continuous school-level or census-tract level covariates for each cluster. In the table, the column designated as "Cluster 0" reports summary statistics for those high schools without any fast food restaurants within one mile of their location.``Median Income'' and ``Proportion of residents...'' refer to characteristics of the population living in the census tract in which schools are located.}
\end{table}
\end{landscape}


\begin{landscape}
\begin{figure}[H]
    \centering
    \includegraphics[width =  1.15\textheight]{figures/map_plot.png}
    \caption{Spatial map of the probability of co-clustering with a reference school denoted by a star. Probabilities are color-coded with lighter colors indicating larger probabilities within each of 2 probability intervals considered, (0,0.5] and (0.5,1]. }
    \label{fig:probmap}
\end{figure}
\end{landscape}


\subsection{Health Outcomes Models}

In discussing the results of our two proposed health outcomes models, we start by providing a description of the schools whose data are used, since the CGLM was fit to a smaller subset of schools.   The proportion of students that are obese is similar in both the schools in the CGLM and BKMR (Table 4), which is encouraging since schools are not excluded on the basis of the outcome in the CGLM. However, schools used to fit the CGLM are less likely to have few FFRs around them - only 7\% have between 1 and 4 FFRs compared to 28 \% in the comparative BKMR dataset. 

\textcolor{Blue}{I think that the text below should be organized by first discussing the results of the CGLM models by itself, the results of the BKMR model by itself and then a comparison of the two models, when we group/average over the schools that belong to the same cluster according to the mode cluster assignment. I would add a sentence that tells the reader that we first discuss the results of the two models separately and then we compare them.} Turning to model results, the estimated effect of each cluster of FFR spatial distributions around a school on the probability of obesity, as yielded by the CGLM, and the estimated effect of a school's spatial pattern of surrounding FFRs on the probability of obesity, as yielded by the BKMR model in (\ref{eqn:outcomes_bkmr}) can be seen in Figure \ref{fig:second_stage_profile}. As the figure shows, we identify a weak association between obesity and cluster assignment in both models, with the strongest protective effect exhibited by cluster 6, the cluster whose density mode is closer to the upper bound of the (0,1) mile interval--i.e., the cluster of schools for which the greatest proportion of FFRs are located farther away from the school. 
Specifically, according to the CGLM, children attending schools consistently assigned to cluster 6 have a 35\%(95\% CI: 33\%,38\%) probability of being overweight or obese, while, for other clusters, the lower bound estimates of the probability of obesity range from 37\% to 40\%. 

\par 
As can be noted from Figure \ref{fig:est_clusters}, the density function representing cluster 6 contains the majority of its mass past 3 quarters of a mile, in explicit contrast to the other clusters which tend to have greater density - and consequently FFRs - closer to the school. This finding is consistent with the substantive expectation that students who are exposed to FFRs in the immediate environment around schools are more likely to be obese than they would be otherwise. 

\par Figure \ref{fig:second_stage_quantity} shows the estimated obesity probability as a function of the number of FFRs within a 1-mile radius of the school, independent of the association between cluster membership and obesity (details on how these probabilities were calculated are available in Section \ref{sec:prob_calc}). The results of the CGLM and the BKRM model are overlaid for comparison. As the figure indicates, there is a rough agreement between the two models with respect to the effect of the number of FFRs on obesity, at least for schools with 2-4 FFRs within one mile of their location. However, there is a marked contrast between the two models as the number of FFRs increase beyond 4, with the CGLM estimating a decreasing probability with higher variance and the BKMR model estimating an increased risk of obesity. We posit that the likely explanation for this stark contrast is due to the different set of schools being included in the analysis for the CGLM. The selection mechanism used to identify the schools that contribute to the estimation in the CGLM induces a selection bias, as schools that have more FFRs around them are more likely to be included in the sample as they are the schools that provide the most information to the cluster estimation and consequently are most likely to be consistently classified. This highlights a weakness of the CGLM approach for this dataset where many schools have few FFRs around them. However, we recognize that this may not represent an issue in datasets or studies where subjects uniformly have moderate to high levels of exposure to a BEF of interest. Finally, comparison of these models to more naive competitor models by WAIC are shown in Supplementary Section Table \ref{tab:prelim_comparison}. Both the BKMR and CGLM perform better by this metric than their naive counterparts.




\begin{table}[H]
\centering
\input{tables/consensus_table}
\caption{Descriptive Statistics for Schools Analyzed in the Consensus GLM. ``Median Income'' and ``Proportion of residents...'' are characteristics of the population living in the census tract where schools are located. IQR = Inter-quartile range; FFR = Fast Food Restaurant. All numerical values for categorical rows are the column percentage within the left row heading. }
\label{tab:conensus}
\end{table}

\begin{figure}[H]
    \centering
    \includegraphics[width = \textwidth]{figures/h_plot.png}
    \caption{Health Outcome Fast Food Restaurant (FFR) Spatial Proximity Effects. Bayesian Kernel Machine Regression (BKMR) random school intercepts 95 \% credible interval are plotted as lines with cluster median dots colored in black. Consensus GLM(CGLM) effects' 95\% credible intervals for each cluster are plotted in brown with triangles denoting the median estimate. The reference dotted line is the posterior mean probability of obesity at a Majority White Sub-Urban High School with at least one FFR within a mile of the school's location.BKMR and CGLM results are estimated from datasets of 1211 and 666 schools, respectively. }
    \label{fig:second_stage_profile}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width = \textwidth]{figures/FFR_QuantityEffect.png}
    \caption{Health Outcome fast food restaurant (FFR) Quantity Effect: Consensus GLM results come from a dataset of  666 schools, while Bayesian Kernel Machine Regression (BKMR) results come from 1211 schools. Reference Line is 1 - or no association. Point ranges represent median and 95\% Credible Intervals}
    \label{fig:second_stage_quantity}
\end{figure}


==> Paper_Sections/SupplementaryMaterial.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width = .85 \textwidth]{figures/cluster_intensities_two.png}
    \caption{Median and 95\% Credible Interval Estimates for cluster normalized intensity functions on transformed $\mathbb{R}$ scale.}
    \label{fig:raw_cluster_intensities}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width = .85 \textwidth]{figures/FFR_spatialeffect_withmode.png}
    \caption{Posterior Mode (MGLM) and Consensus GLM (CGLM) analyses. Results show the school's proportion of obese students within each cluster configuration.}
    \label{fig:mode_glm_comp}
\end{figure}

\begin{table}[H]
    \centering
    \input{tables/prelim_comparison}
    \caption{Widely Applicable Information Criterion (WAIC) for Traditional (T) models 1-3, Bayesian Kernel Machine Regression (BKMR) and Consensus GLM (CGLM) for both Reduced and Full datasets corresponding to ``In Consensus'' and ``All'' columns from Table \ref{tab:conensus}, respectively. Each model contains the same adjusting covariates and different measures of FFR exposure in a logistic regression modeling 9th grader obesity. T. 1 includes the \# of FFR within 1 mile of the school. T. 2 includes the distance to the closest FFR and T. 3 includes both the previous measures. CGLM and BKMR are as denoted in the text. }
    \label{tab:prelim_comparison}
\end{table}


\begin{table}[H]
    \centering
    \input{tables/extra_descriptives}
    \caption{Supplemental School Covariate Information. The lower half of the table contains the column percentage of schools that are either Chartered or traditional.}
    \label{tab:supp_descriptive}
\end{table}

==> tables/cluster_table.tex <==
\begin{tabular}{llcccccccc}
\toprule
& & \multicolumn{7}{c}{Mode Cluster} & \multicolumn{1}{c}{} \\ 
 &  & 0 & 1 & 2 & 3 & 4 & 5 & 6 & \multicolumn{1}{c}{Total} \\ 
 & & (n=446) & (n=258) & (n=106) & (n=31) & (n=30) & (n=234) & (n=106) & (n=1211) \\
\midrule
Majority Race & African American &  $\phantom{0}2$ & $\phantom{0}2$ & $\phantom{0}3$ & $\phantom{0}1$ & $\phantom{0}0$ & $\phantom{0}0$ & $\phantom{0}3$ & $\phantom{0}1$ \\
 & Asian &  $\phantom{0}2$ & $\phantom{0}6$ & $\phantom{0}3$ & $\phantom{0}4$ & $\phantom{0}4$ & $\phantom{0}5$ & $\phantom{0}3$ & $\phantom{0}4$ \\
 & Hispanic &  $27$ & $37$ & $27$ & $26$ & $29$ & $30$ & $16$ & $28$ \\
 & No Majority &  $11$ & $13$ & $13$ & $14$ & $18$ & $13$ & $19$ & $13$ \\
 & White &  $59$ & $42$ & $53$ & $55$ & $49$ & $52$ & $58$ & $54$ \\
Urbanicity & Rural &  $39$ & $\phantom{0}9$ & $13$ & $13$ & $\phantom{0}9$ & $\phantom{0}6$ & $19$ & $21$ \\
 & Sub-Urban &  $34$ & $42$ & $37$ & $44$ & $43$ & $45$ & $42$ & $40$ \\
 & Urban &  $27$ & $49$ & $50$ & $42$ & $47$ & $48$ & $39$ & $39$ \\
FFR Quantity & [1,4] &  $\phantom{0}0$ & $41$ & $37$ & $49$ & $35$ & $47$ & $55$ & $28$ \\
 & $\geq$5 &  $\phantom{0}0$ & $59$ & $63$ & $51$ & $65$ & $53$ & $45$ & $35$ \\
 & Zero &  $100$ & $\phantom{0}0$ & $\phantom{0}0$ & $\phantom{0}0$ & $\phantom{0}0$ & $\phantom{0}0$ & $\phantom{0}0$ & $37$ \\
%Median Income (1000 USD) & Median (Q1-Q3)  & 53.8 (41.8-73.9) & 55.2 (43.9-76.6) & 52.5 (44.9-73.5) & 60.5 (43.9-82.7) & 68.9 (49-90.6) & 60.9 (46.8-77) & 67.4 (43.4-86.5) & 58.2 (43.9-78.4) \\
Median HH Income (1000 USD) & Median   & 53.8 & 55.2   & 52.5  & 60.5  & 68.9  & 60.9   & 67.4  & 58.2   \\
of residents in schools' CT &(Q1-Q3)  &  (41.8-73.9) &  (43.9-76.6) &  (44.9-73.5) & (43.9-82.7) & (49-90.6) &  (46.8-77) &  (43.4-86.5) &  (43.9-78.4) \\
                            & IQR  & $32$ & $32.7$ & $28.6$ & $38.8$ & $41.5$ & $30.1$ & $43.0$ & $34.5$ \\
Proportion of adults & Median & 24.9  & 24.9  & 25.2  & 25.4  & 25.6  & 25.3  & 25.5  & 25.1  \\
with $\geq$ 16 years of education & (Q1-Q3) & (24.1-26.1) & (24.2-27) & (24.1-27.3) & (24.4-27) & (24.3-27.1) & (24.1-26.6) &  (24.5-26.9) & (24.2-26.6) \\
  & IQR  & $\phantom{0}2$ & $\phantom{0}2.8$ & $\phantom{0}3.3$ & $\phantom{0}2.6$ & $\phantom{0}2.8$ & $\phantom{0}2.5$ & $\phantom{0}2.5$ & $\phantom{0}2.4$ \\
\bottomrule
\end{tabular}


==> tables/consensus_table.tex <==
\begin{tabular}{llccc}
\hline
 &  &   In Consensus & Not in Consensus & \multicolumn{1}{c}{All} \\ 
\hline
Majority Race & African American &  $\phantom{0}1$ & $\phantom{0}1$ & $\phantom{0}1$ \\
 & Asian &  $\phantom{0}5$ & $\phantom{0}4$ & $\phantom{0}4$ \\
 & Hispanic &  $30$ & $28$ & $29$ \\
 & No Majority &  $16$ & $13$ & $14$ \\
 & White &  $48$ & $53$ & $52$ \\
Urbanicity & Rural &  $\phantom{0}8$ & $11$ & $10$ \\
 & Sub-Urban &  $35$ & $47$ & $44$ \\
 & Urban &  $57$ & $42$ & $46$ \\
FFR Quantity & [1,4] &  $21$ & $54$ & $45$ \\
 & $\geq$5 &  $79$ & $46$ & $55$ \\
\hline 
Proportion Obese & Median (Q1-Q3)  & 40.9 (33.3-47.4) & 41.3 (34.1-48.2) & 41.3 (33.9-48) \\
 & IQR  & $15.4$ & $13.9$ & $14.5$ \\
Median Income (1000 USD) & Median (Q1-Q3)  & 58.5 (42.5-78) & 61.1 (46.1-81.9) & 60.8 (45-80.4) \\
 & IQR  & $35.6$ & $35.8$ & $35.4$ \\
Proportion of residents  & Median (Q1-Q3)  & 25.3 (24.2-26.7) & 25.4 (24.2-26.9) & 25.4 (24.2-26.8) \\
 with $\geq$ 16 years of education & IQR  & $\phantom{0}2.5$ & $\phantom{0}2.7$ & $\phantom{0}2.6$ \\
\hline 
\end{tabular}


==> tables/descriptivetable.tex <==
\begin{tabular}{llccc}
\toprule
 &  & \multicolumn{2}{c}{Subset of schools with} & \multicolumn{1}{c}{All schools} \\
 &  &  $\geq 1$ FFR nearby & no FFRs nearby & \\ \toprule
\multicolumn{1}{l}{\underline{Children}}\\ 
Number       &  & 298,903 & 121,182 & 420,085 \\
$\%$ Obese   &  &  40$\%$$^{\star}$  & 40$\%$  & 40$\%$ \\
\midrule
\multicolumn{1}{l}{\underline{Schools}}\\ 
Number & & 782 & 446 & 1,228 \\
Urbanicity & Rural &  $10$ & $39$ & $20$ \\
 & Sub-Urban &  $44$ & $34$ & $41$ \\
 & Urban &  $46$ & $27$ & $39$ \\
Majority Race & African American &  $\phantom{0}1$ & $\phantom{0}2$ & $\phantom{0}1$ \\
 & Asian &  $\phantom{0}4$ & $\phantom{0}2$ & $\phantom{0}4$ \\
 & Hispanic &  $29$ & $27$ & $28$ \\
 & No Majority &  $14$ & $11$ & $13$ \\
 & White &  $52$ & $59$ & $54$ \\
Median household income (\$1,000 USD)  & Median (Q1-Q3)  & 59.1 (43.4-78.6) & 52.2 (40.2-72.3) & 56.6 (42.3-76.7) \\
of residents  in school's census tract & IQR  & $35.24$ & $32.05$ & $34.4$ \\
Proportion of residents  & Median (Q1-Q3)  & 23.7 (12.6-38.6) & 19.2 (11.2-31.7) & 21.7 (12-36) \\
with $\geq$ 16 years of education & IQR  & $26.0$ & $20.5$ & $24.0$ \\
FFR Quantity & 0 &  $\phantom{0}0$ & $100$ & $36$ \\
 & [1,4] &  $44$ & $\phantom{0}0$ & $28$ \\
 & $\geq$5 &  $56$ & $\phantom{0}0$ & $35$ \\
 Closest FFR (Miles) & Median (Q1-Q3)  & 0.4 (0.3-0.6) & - & 0.4 (0.3-0.6) \\
 & IQR  & $\phantom{0}0.4$ & - & $\phantom{0}0.4$ \\
\bottomrule
\end{tabular}


==> tables/extra_descriptives.tex <==
\begin{tabular}{llccc}
\hline
 &  & $\geq 1$ FF & no FFRs nearby & \multicolumn{1}{c}{All schools} \\ 
\hline
\% Receiving Free   & Median (Q1-Q3)  & 48.9 (26.1-68) & 48.9 (27.6-71.9) & 48.9 (26.9-68.8) \\
 or Reduced Price Meals & IQR  & $41.9$ & $44.2$ & $42$ \\
\hline 
Traditional High School & & $78.13$ & $78.25$ & $78.18$ \\
Charter High School & & $21.87$ & $21.75$ & $21.82$ \\
\hline 
\end{tabular}

==> tables/pi_table.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue May 26 11:51:59 2020
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrr}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
Median (\%) & 15 & 6 & 24 & 18 & 29 & 7 \\ 
  IQR (\%) & 3 & 2 & 4 & 5 & 5 & 2 \\ 
   \hline
\end{tabular}
\caption{Nonzero Cluster Probabilities} 
\end{table}


==> tables/prelim_comparison.tex <==

\centering
\begin{tabular}{lll}
  \hline
Models & Full & Reduced \\ 
  \hline
T.1 & 30,566.95 & 12,217.12 \\ 
  T.2 & 33,972.94 & 17,040.08 \\ 
  T.3 & 26,096.42 & 12,169.42 \\ 
  BKMR & 13,315.55 & 10,552.55 \\ 
  CGLM & - & 9,883.43 \\ 
   \hline
\end{tabular}

